A Quality Index Metric and Method for Online Self-Assessment of Autonomous Vehicles Sensory Perception

Reliable object detection using cameras plays a crucial role in enabling autonomous vehicles to perceive their surroundings. However, existing camera-based object detection approaches for autonomous driving lack the ability to provide comprehensive feedback on detection performance for individual frames. To address this limitation, we propose a novel evaluation metric, named as the detection quality index (DQI), which assesses the performance of camera-based object detection algorithms and provides frame-by-frame feedback on detection quality. The DQI is generated by combining the intensity of the fine-grained saliency map with the output results of the object detection algorithm. Additionally, we have developed a superpixel-based attention network (SPA-NET) that utilizes raw image pixels and superpixels as input to predict the proposed DQI evaluation metric. To validate our approach, we conducted experiments on three open-source datasets. The results demonstrate that the proposed evaluation metric accurately assesses the detection quality of camera-based systems in autonomous driving environments. Furthermore, the proposed SPA-NET outperforms other popular image-based quality regression models. This highlights the effectiveness of the DQI in evaluating a camera's ability to perceive visual scenes. Overall, our work introduces a valuable self-evaluation tool for camera-based object detection in autonomous vehicles.

==> nomenclature.tex <==
\section*{Nomenclature}
\addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$V_1,V_2,V_3$}]

\item[B-IQA] Blind Image Quality Assessment
\item[BRISQUE] Blind/Referenceless Image Spatial Quality Evaluator
\item[CNN] Convolutional Neural Network
\item[CSP] Cross-Stage Partial Connections
\item[DIIVINE] Distortion Identification-based Image Verity and Integrity Evaluation
\item[DQI] Detection Quality Index
\item{IoU} Intersection Over Union
\item{IMU} Inertial Measurement Unit
\item{mAP} Mean Average Precision
\item[MLP] Multi-Layer Perceptron Network
\item{PLCC} Pearson's Linear Correlation Coefficient
\item{R2} R-Square
\item[R-CNN] Rich Feature Hierarchies Convolutional Neural Network
\item{SLIC} Simple Linear Ietrative Clustering
\item[SOTA] State of the Art Algorithms
\item[SPA-NET] SuperPixel-based Attention Neural Network
\item[SPP] Spatial Pyramid Pooling
\item{SRCC} Spearman Rank-Order Correlation Coefficient
\item[ViT] Visual Transformer 
\item[YOLO] You Look Only Once Object Detection Algorithm








\end{IEEEdescription}
